Improved theoretical guarantees regarding a class of two-row cutting planes

The corner polyhedron is described by minimal valid inequalities from maximal lattice-free convex sets. For the Relaxed Corner Polyhedron (RCP) with two free integer variables and any number of non-negative continuous variables, it is known that such facet defining inequalities arise from maximal lattice-free splits, triangles and quadrilaterals. We improve on the tightest known upper bound for the approximation of the RCP, purely by minimal valid inequalities from maximal lattice-free quadrilaterals, from 2 to 1.71. We generalize the tightest known lower bound of 1.125 for the approximation of the RCP, purely by minimal valid inequalities from maximal lattice-free triangles, to an infinite subclass of quadrilaterals.

==> formatfig.tex <==

%\include{BoxedEPS}
%\SetOzTeXEPSFSpecial
\newlength{\tmpLength}
%\HideDisplacementBoxes

\newcommand{\oneWidth}[3][0]{
  \setlength{\tmpLength}{0.99\textwidth}
  \setlength{\tmpLength}{#3\tmpLength}
  \centerline{
    \includegraphics[angle=#1,width=\tmpLength]{#2}
    \vspace{-12pt}
  } % centering
}

\newcommand{\oneWidthLabel}[4][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{#3\tmpLength}
  \centerline{
    \begin{tabular}{c}
      \includegraphics[angle=#1,width=\tmpLength]{#2} \\
      \small \mbox{#4}
    \end{tabular}
  } % centering
}

\newcommand{\oneHeight}[3][0]{
  \setlength{\tmpLength}{0.9\textheight}
  \setlength{\tmpLength}{#3\tmpLength}
	    {
	      \centering
	      \includegraphics[angle=#1,height=\tmpLength]{#2}
	    } % centering
}

\newcommand{\twoWidth}[3][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.5\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} \\
      \small \mbox{(a)}
      &
      &
      \small \mbox{(b)}
    \end{tabular}
  } % centering
}

\newcommand{\twoHeight}[3][0]{
  \setlength{\tmpLength}{0.95\textheight}
  \setlength{\tmpLength}{0.28\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[angle=#1,height=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#3} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
    \end{tabular}
  } % centering
}

\newcommand{\twoHeightLabels}[5][0]{
  \setlength{\tmpLength}{0.95\textheight}
  \setlength{\tmpLength}{0.33\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[angle=#1,height=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#3} \\
      \small \mbox{#4}
      &
      \small \mbox{#5}
    \end{tabular}
  } % centering
}

\newcommand{\twoHeightLabelsAnother}[5][0]{
  \setlength{\tmpLength}{0.95\textheight}
  \setlength{\tmpLength}{0.44\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[angle=#1,height=0.9\tmpLength]{#2}
      &
      \includegraphics[angle=#1,height=1.2\tmpLength]{#3} \\
      \small \mbox{#4}
      &
      \small \mbox{#5}
    \end{tabular}
  } % centering
}

\newcommand{\twoHeightLabelsYetAnother}[5][0]{
  \setlength{\tmpLength}{0.95\textheight}
  \setlength{\tmpLength}{0.44\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[angle=#1,height=1.1\tmpLength]{#2}
      &
      \includegraphics[angle=#1,height=1.2\tmpLength]{#3} \\
      \small \mbox{#4}
      &
      \small \mbox{#5}
    \end{tabular}
  } % centering
}

\newcommand{\sixTwoAcrossTall}[7][0]{
  \setlength{\tmpLength}{0.9\textheight}
  \setlength{\tmpLength}{0.33\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[angle=#1,height=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#3} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)} \\
      \includegraphics[angle=#1,height=\tmpLength]{#4}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#5} \\
      \small \mbox{(c)}
      &
      \small \mbox{(d)} \\
      \includegraphics[angle=#1,height=\tmpLength]{#6}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#7} \\
      \small \mbox{(e)}
      &
      !\small \mbox{(f)} 
    \end{tabular}
  } % centering
}

\newcommand{\twoWidthLabels}[5][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.50\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} \\
      \small \mbox{#4}
      &
      &
      \small \mbox{#5}
    \end{tabular}
  } % centering
}

\newcommand{\twoAcross}[3][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.33\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} 
      \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
    \end{tabular}
  } % centering
}

\newcommand{\twoAcrossLabels}[5][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.5\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3}
      \\
      \small \mbox{#4}
      &
      \small \mbox{#5}
    \end{tabular}
  } % centering
}

\newcommand{\twoAcrossLabelsLarger}[5][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.32\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3}
      \\
      \small \mbox{#4}
      &
      \small \mbox{#5}
    \end{tabular}
  } % centering
}

\newcommand{\twoAcrossZoomFirst}[6]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.5\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#5}
      &
      \includegraphics[width=\tmpLength]{#6} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
    \end{tabular}
  } % centering
}

\newcommand{\twoAcrossZoomAll}[6]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.5\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#5}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#6} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
    \end{tabular}
  } % centering
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%            ACROSS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\threeAcrossZoomFirst}[7]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#5}
      &
      \includegraphics[width=\tmpLength]{#6}
      &
      \includegraphics[width=\tmpLength]{#7} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
      &
      \small \mbox{(c)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossZoomFirstHeight}[8][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpWidth }{0.25\tmpLength}
  \setlength{\tmpHeight}{#8\tmpWidth}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[viewport=#1 #2 #3 #4, ,width=\tmpWidth,height=\tmpHeight]{#5}
      &
      \includegraphics[viewport=#1 #2 #3 #4, ,width=\tmpWidth,height=\tmpHeight]{#6} 
      &
      \includegraphics[viewport=#1 #2 #3 #4, ,width=\tmpWidth,height=\tmpHeight]{#7} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
      &
      \small \mbox{(c)}
    \end{tabular}
  } % centering 
}


\newcommand{\twoAcrossZoomLastLabels}[8]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.5\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[width=\tmpLength]{#5}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#6} \\
      \small \mbox{(#7)}
      &
      \small \mbox{(#8)}
    \end{tabular}
  } % centering
}


\newcommand{\fourTwoAcross}[5][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.5\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)} \\
      \includegraphics[angle=#1,width=\tmpLength]{#4}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#5} \\
      \small \mbox{(c)}
      &
      \small \mbox{(d)} 
    \end{tabular}
  } % centering
}

\newcommand{\threeAcross}[4][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      \vspace{-1pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} 
      \vspace{-1pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#4}
      \vspace{-1pt} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
      &
      \small \mbox{(c)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossHeight}[5][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{#5\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[angle=#1,height=\tmpLength]{#2}
      \vspace{-1pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#3} 
      \vspace{-1pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#4}
      \vspace{-1pt} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
      &
      \small \mbox{(c)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossZoomAllABC}[7]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#5}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#6}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#7} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
      &
      \small \mbox{(c)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossZoomAllDEF}[7]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#5}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#6}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#7} \\
      \small \mbox{(d)}
      &
      \small \mbox{(e)}
      &
      \small \mbox{(f)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossZoomAllGHI}[7]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#5}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#6}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#7} \\
      \small \mbox{(g)}
      &
      \small \mbox{(h)}
      &
      \small \mbox{(i)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossZoomLastTwoABC}[9]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[width=\tmpLength]{#9}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#9}
      &
      \includegraphics*[viewport=#5 #6 #7 #8, width=\tmpLength]{#9} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
      &
      \small \mbox{(c)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossZoomLastTwoDEF}[9]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[width=\tmpLength]{#9}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#9}
      &
      \includegraphics*[viewport=#5 #6 #7 #8, width=\tmpLength]{#9} \\
      \small \mbox{(d)}
      &
      \small \mbox{(e)}
      &
      \small \mbox{(f)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossZoomLastABC}[7]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[width=\tmpLength]{#5}
      &
      \includegraphics[width=\tmpLength]{#6}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#7} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
      &
      \small \mbox{(c)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossZoomLastDEF}[7]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[width=\tmpLength]{#5}
      &
      \includegraphics[width=\tmpLength]{#6}
      &
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#7} \\
      \small \mbox{(d)}
      &
      \small \mbox{(e)}
      &
      \small \mbox{(f)}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossLabels}[7][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.33\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      \vspace{-1pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} 
      \vspace{-1pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#4}
      \vspace{-1pt} \\
      \small \mbox{#5}
      \vspace{-1pt}
      &
      \small \mbox{#6}
      \vspace{-1pt}
      &
      \small \mbox{#7}
      \vspace{-1pt}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossLabelsSmaller}[7][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.30\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#4} \\
      \small \mbox{#5}
      &
      \small \mbox{#6}
      &
      \small \mbox{#7}
    \end{tabular}
  } % centering
}

\newcommand{\threeAcrossLabelsSmall}[7][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.26\tmpLength}
  \centerline{
    \begin{tabular}{ccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} 
      &
      \includegraphics[angle=#1,width=\tmpLength]{#4} \\
      \small \mbox{#5}
      &
      \small \mbox{#6}
      &
      \small \mbox{#7}
    \end{tabular}
  } % centering
}

\newcommand{\fourAcross}[5][0]{
  \setlength{\tmpLength}{0.97\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{cccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} 
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#4} 
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#5}
      \vspace{-1pt} \\
      \small \mbox{(a)}
      \hspace{-4pt}
      &
      \small \mbox{(b)}
      \hspace{-4pt}
      &
      \small \mbox{(c)}
      \hspace{-4pt}
      &
      \small \mbox{(d)}
    \end{tabular}
  } % centering
}

\newcommand{\fourAcrossNoLabels}[5][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.24\tmpLength}
  \centerline{
    \begin{tabular}{cccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} 
      &
      \includegraphics[angle=#1,width=\tmpLength]{#4} 
      &
      \includegraphics[angle=#1,width=\tmpLength]{#5} \\
    \end{tabular}
  } % centering
}

\newcommand{\fourAcrossLabels}[9][0]{
  \setlength{\tmpLength}{0.97\textwidth}
  \setlength{\tmpLength}{0.25\tmpLength}
  \centerline{
    \begin{tabular}{cccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} 
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,width=0.30\tmpLength]{#4}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,width=0.2625\tmpLength]{#5}
      \vspace{-1pt} \\
      \small \mbox{#6}
      \hspace{-4pt}
      &
      \small \mbox{#7}
      \hspace{-4pt}
      &
      \small \mbox{#8}
      \hspace{-4pt}
      &
      \hspace {6pt}
      \small \mbox{#9}
    \end{tabular}
  } % centering
}

\newcommand{\fourAcrossLabelsHeight}[9]{
  \setlength{\tmpLength}{0.97\textwidth}
  \setlength{\tmpLength}{0.24\tmpLength}
  \centerline{
    \begin{tabular}{cccc}
      \includegraphics[height=#9\tmpLength]{#1}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \includegraphics[height=#9\tmpLength]{#2}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \includegraphics[height=#9\tmpLength]{#3}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \includegraphics[height=#9\tmpLength]{#4}
      \vspace{-1pt} \\
      \small \mbox{#5}
      \hspace{-4pt}
      &
      \small \mbox{#6}
      \hspace{-4pt}
      &
      \small \mbox{#7}
      \hspace{-4pt}
      &
      \small \mbox{#8}
    \end{tabular}
  } % centering
}

\newcommand{\fourAcrossLabelsSmaller}[9][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.21\tmpLength}
  \centerline{
    \begin{tabular}{cccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3} 
      &
      \includegraphics[angle=#1,width=\tmpLength]{#4} 
      &
      \includegraphics[angle=#1,width=\tmpLength]{#5} \\
      \small \mbox{#6}
      &
      \small \mbox{#7}
      &
      \small \mbox{#8}
      &
      \small \mbox{#9}
    \end{tabular}
  } % centering
}

\newcommand{\fourAcrossLabelsSpace}[9][0]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.225\tmpLength}
  \centerline{
    \begin{tabular}{cccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3}
      \hspace {15 pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#4}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#5} \\
      \small \mbox{#6}
      &
      \small \mbox{#7}
      \hspace {15 pt}
      &
      \small \mbox{#8}
      &
      \small \mbox{#9}
    \end{tabular}
  } % centering
}

\newcommand{\fourAcrossZoomFirst}[8]{
  \setlength{\tmpLength}{0.95\textwidth}
  \setlength{\tmpLength}{0.22\tmpLength}
  \centerline{
    \begin{tabular}{cccc}
      \includegraphics*[viewport=#1 #2 #3 #4, width=\tmpLength]{#5}
      &
      \includegraphics[width=\tmpLength]{#6}
      &
      \includegraphics[width=\tmpLength]{#7}
      &
      \includegraphics[width=\tmpLength]{#8} \\
      \small \mbox{(a)}
      &
      \small \mbox{(b)}
      &
      \small \mbox{(c)}
      &
      \small \mbox{(d)}
    \end{tabular}
  } % centering
}

\newcommand{\fiveAcross}[6][0]{
  \setlength{\tmpLength}{0.98\textwidth}
  \setlength{\tmpLength}{0.19\tmpLength}
  \centerline{
    \begin{tabular}{ccccc}
      \includegraphics[angle=#1,width=\tmpLength]{#2}
      \vspace{-0.5pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#3}
      \vspace{-0.5pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#4}
      \vspace{-0.5pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#5}
      \vspace{-0.5pt}
      &
      \includegraphics[angle=#1,width=\tmpLength]{#6}
      \vspace{-1pt} \\
      \small \mbox{(a)}
      \vspace{-1pt}
      &
      \small \mbox{(b)}
      \vspace{-1pt}
      &
      \small \mbox{(c)}
      \vspace{-1pt}
      &
      \small \mbox{(d)}
      \vspace{-1pt}
      &
      \small \mbox{(e)}
      \vspace{-1pt}
    \end{tabular}
  } % centering
}

\newcommand{\fiveAcrossHeight}[7][0]{
  \setlength{\tmpLength}{0.98\textwidth}
  \setlength{\tmpLength}{#7\tmpLength}
  \centerline{
    \begin{tabular}{ccccc}
      \includegraphics[angle=#1,height=\tmpLength]{#2}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#3}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#4}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#5}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#6}
      \vspace{-1pt} \\
      \small \mbox{(a)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(b)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(c)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(d)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(e)}
      \vspace{-1pt}
    \end{tabular}
  } % centering
}

\newcommand{\sixAcrossHeight}[7][0]{
  \setlength{\tmpLength}{0.98\textwidth}
  \setlength{\tmpLength}{0.165\tmpLength}
  \centerline{
    \begin{tabular}{cccccc}
      \includegraphics[angle=#1,height=\tmpLength]{#2}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#3}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#4}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#5}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=1.11\tmpLength]{#6}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=1.21\tmpLength]{#7}
      \vspace{-1pt} \\
      \small \mbox{(a)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(b)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(c)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(d)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(e)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(f)}
      \vspace{-1pt}
    \end{tabular}
  } % centering
}

\newcommand{\sixAcrossHeightAnother}[7][0]{
  \setlength{\tmpLength}{0.98\textwidth}
  \setlength{\tmpLength}{0.1575\tmpLength}
  \centerline{
    \begin{tabular}{cccccc}
      \includegraphics[angle=#1,height=\tmpLength]{#2}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#3}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#4}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=\tmpLength]{#5}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=0.9\tmpLength]{#6}
      \vspace{-0.5pt}
      \hspace{-4pt}
      &
      \includegraphics[angle=#1,height=1.2\tmpLength]{#7}
      \vspace{-1pt} \\
      \small \mbox{(f)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(g)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(h)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(i)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(j)}
      \vspace{-1pt}
      \hspace{-4pt}
      &
      \small \mbox{(k)}
      \vspace{-1pt}
    \end{tabular}
  } % centering
}

%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%

\newcommand{\threeDownTwoColumns}[6]{
  \setlength{\tmpLength}{0.45\textwidth}
  \setlength{\tmpLength}{0.50\tmpLength}
    \centerline{
    \begin{tabular}{cc}
      \includegraphics[width=\tmpLength]{#1}
      &
      \includegraphics[width=\tmpLength]{#2} \\
      \small \mbox{(a)}
      &	
      \small \mbox{(b)} \\
      \includegraphics[width=\tmpLength]{#3}
      &
      \includegraphics[width=\tmpLength]{#4} \\
      \small \mbox{(c)}
      &
      \small \mbox{(d)} \\
      \includegraphics[width=\tmpLength]{#5}
      &
      \includegraphics[width=\tmpLength]{#6} \\
      \small \mbox{(e)}
      &
      \small \mbox{(f)}
    \end{tabular}
    } % centering
}

\newcommand{\oneAcrossTwoColumnsLabel}[2]{
  \setlength{\tmpLength}{0.45\textwidth}
  \setlength{\tmpLength}{0.50\tmpLength}
  \centerline{
    \begin{tabular}{c}
      \includegraphics[width=\tmpLength]{#1} \\
      \small \mbox{#2}
    \end{tabular}
  } % centering
}

\newcommand{\twoAcrossTwoColumnsLabels}[4]{
  \setlength{\tmpLength}{0.45\textwidth}
  \setlength{\tmpLength}{0.50\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[width=\tmpLength]{#1}
      &
      \includegraphics[width=\tmpLength]{#2} \\
      \small \mbox{#3}
      &
      \small \mbox{#4}
    \end{tabular}
  } % centering
}

\newcommand{\twoAcrossTwoColumnsLabelsZoom}[8]{
  \setlength{\tmpLength}{0.45\textwidth}
  \setlength{\tmpLength}{0.50\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics*[viewport=#1 #2 #3 #4,width=\tmpLength]{#5}
      &
      \includegraphics*[viewport=#1 #2 #3 #4,width=\tmpLength]{#6} \\
      \small \mbox{#7}
      &
      \small \mbox{#8}
    \end{tabular}
  } % centering
}

\newcommand{\twoAcrossTwoColumnsLabelsZoomLast}[8]{
  \setlength{\tmpLength}{0.45\textwidth}
  \setlength{\tmpLength}{0.50\tmpLength}
  \centerline{
    \begin{tabular}{cc}
      \includegraphics[width=\tmpLength]{#5}
      &
      \includegraphics*[viewport=#1 #2 #3 #4,width=\tmpLength]{#6} \\
      \small \mbox{#7}
      &
      \small \mbox{#8}
    \end{tabular}
  } % centering
}

